A discrete-time temporal deontic STIT logic based on interpreted systems

We present a STIT ('see to it that') logic with discrete temporal operators and deontic operators in which we can formalize and reason about legal concepts such as persistent duty and the dynamic concept of power from Hohfeld. As our main technical contribution, we show that this logic is sound and complete with respect to the semantics based on interpreted systems and is decidable.

==> trash.tex <==


\newpage
\topskip0pt
\vspace*{\fill}
\textbf{Old stuff begins here}
\vspace*{\fill}
\newpage

\subsection{A relational semantics for deontic temporal STIT logic}

$DTS^U$ interpreted systems are intuitive models when formalising agents' actions, duties and the effects of agents' choices on paths of histories. Note that, in our interpreted systems, we are only concerned with discrete time.


\begin{definition}\emph{($DTS^U$ interpreted system)}\label{def2}
A $DTS^U$ interpreted system is defined as a tuple  $\mathcal{I}=(H, R_\Box, \{R_{[i]} \mid i \in Agt\}, R_{\mathsf{Agt}}, \{R_{\mathsf{O}_i}\mid i\in Agt\},V)$ s.t.:

\begin{itemize}
\item $H$ is a set of histories;
\item $R_\Box, R_{[i]}, R_{\mathsf{Agt}} \subseteq (H \times \mathbb{N})^2$ are equivalence relations s.t.:

\begin{enumerate}

    \item[\textbf{(D1)}]  if $(h, t)R_\Box(h', s)$ then $t= s$;
    \item[\textbf{(D2)}] $R_{[i]} \subseteq R_\Box$;
    \item[\textbf{(D3)}] $R_\Box((h, t+1)) \subseteq \{(h', t+1) \mid (h', t) \in R_{\mathsf{Agt}}((h, t))\}$;
    
    \item[\textbf{(D4)}]for all $(h,t), (h_i,t_i)\in (H\times\mathbb{N})^2$, where $i\in Agt$, if $(h_i,t_i) \in R_\Box((h,t))$ for all $i$, then \\$\bigcap_{i\in Agt} R_{[i]}((h_i,t_i))\ne\emptyset$;
    
    \item[\textbf{(D5)}]  $R_{\mathsf{Agt}}((h,t)) = \bigcap_{i \in Agt}R_{[i]}((h,t))$.

\end{enumerate}
\item For all $i\in Agt$ and $w,v,u\in H\times\mathbb{N}$, $R_{\mathsf{O}_i}\subseteq (H\times \mathbb{N})^2$ are relations s.t.:
 \begin{enumerate}
        \item[\textbf{(D6)}]$R_{\mathsf{O}_i}\subseteq R_{\Box}$;
        

        \item[\textbf{(D7)}]$R_{\mathsf{O}_i}$ is serial;
    
        \item[\textbf{(D8)}] if $R_{\mathsf{O}_i}wv$ and $R_{[i]}vu$ then $R_{\mathsf{O}_i}wu$;
    
        \item[\textbf{(D9)}]
        if $R_{\Box}wv$ and $R_{\mathsf{O}_i}vu$, then $R_{\mathsf{O}_i}wu$.
   \end{enumerate}
\item $V: P\to\mathcal{P}(H\times\mathbb{N})$ is a valuation function for atomic formulas, where $P$ is the set of propositional letters.
\end{itemize}
\end{definition}

Interpreted systems are indeed relational models with possible worlds represented by tuples in the form of $(h,t)$. A history $h$ can be seen as a maximal set of linearly ordered possible worlds, representing some complete temporal evolution of a world. For the possible world $(h,t)$, the first element $h$ means that the world is in the history $h$, and the second element $t$ means that the world is in the $t$-th time point after the starting point of $h$. $R_\Box((h,t))$ is the set of worlds that are in the same moment as the world $(h,t)$, and the equivalence classes induced by $R_\Box$ are exactly all the moments (\cite{prior1967past}, \cite{thomason1984combinations}, \cite{zanardo1996branching}). The Constraint \textbf{(D1)} indicates that, a moment is, given the history, what is possible now. For each $(h',s)$ in a moment $R_\Box((h,t))$, we refer to $R_{[i]}((h',s))$ as a choice-cell for agent $i$ at moment $R_\Box((h,t))$. \textbf{(D2)} ensures that $R_{[i]}$ is an equivalence relation partitioning the equivalence classes of $R_\Box$. Similarly, the Constraint \textbf{(D6)} ensures that $R_{\mathsf{O}_i}$ is also a relation contained in $R_\Box$. So the worlds in which all of $i$'s duties are fulfilled accessible from a world $(h,t)$ are confined to the moment $R_\Box((h,t))$, i.e., they neither lie in the future nor in the past. The constraint \textbf{(D3)} corresponds to the STIT principle of no choice between undivided histories: if two histories are undivided at the next moment, then no possible choice for any agent at the current moment distinguishes between the two histories. \textbf{(D4)} expresses exactly the independence of agents condition for STIT logic, which requires that: for each moment and for each way of selecting one possible choice in that moment for each agent $i$,
the intersection of the choices selected by all the agents must contain at least one possible world. In short, simultaneous choices are independent. \textbf{(D5)} guarantees that all agents acting is a sufficient and necessary condition for the whole group of agents acting.
\textbf{(D7)} ensures that every world can reach a world in which $i$ carries out all her duties from the perspective of the current world. \textbf{(D8)} captures the idea that, no choice contains worlds in which $i$ fulfills her duties and in which $i$ doesn't. The constraint \textbf{(D9)} expresses that for each agent, if a world is ideal (in the sense of $i$ fulfills her duties) from the perspective of a particular world in a moment, then, that world is ideal from the perspective of any world in that moment.

A simplified $DTS^U$ interpreted system is given in Figure \ref{interpreted system}, in which $Agt=\{i,j\}, H=\{h_1,h_2,h_3,\\ h_4,...\}$, and $R_{\mathsf{Agt}},\{R_{\mathsf{O}_i}\mid i\in Agt\}$ are not drawn. 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.48\textwidth]{fig/is.pic.jpg}
%    \caption{A Simplified $DTS^U$ Interpreted System}
%    \label{interpreted system}
%\end{figure}


\begin{definition}\emph{($DTS^U$ super-additive interpreted system)} A $DTS^U$ super-additive interpreted system is defined as a tuple 
$\mathcal{I}=(H, R_\Box, \{R_{[i]} \mid i \in Agt\}, R_{\mathsf{Agt}}, \{R_{\mathsf{O}_i}\mid i\in Agt\}, V)$  satisfying all the requirements in Definition \ref{def2} except \textbf{(D5)}, and:
    \begin{enumerate}
        \item[\textbf{(D5*)}]$R_{Agt} ((h,t))\subseteq \bigcap_{i \in Agt}R_{[i]}((h,t))$
        
    \end{enumerate}

\end{definition}
While the constraint \textbf{(D5*)} can be captured by a formula (the axiom \textbf{($i\to Agt$)} in Definition \ref{axiom}), \textbf{(D5)} cannot. Therefore, in order to prove the completeness of our axiomatic system given in Subsection 2.3, we need to firstly prove its completeness w.r.t. $DTS^U$ super-additive interpreted systems, then we show that $\mathfrak{L}_{DTS^U}$ does not distinguish the semantics in terms of $DTS^U$ interpreted systems from the semantics
in terms of $DTS^U$ super-additive interpreted systems. That is to say, the set of validities
w.r.t. the class of $DTS^U$ interpreted systems is equal to the set of validities
w.r.t. the class of super-additive ones.




\begin{definition}{(The logic $\mathsf{DTS^U}$)}
    $\mathsf{DTS^U}$ is the set of validities in the class of $DTS^U$ interpreted systems.
\end{definition}



Now we provide some brief examples to illustrate the expressive power of the language.
\begin{example}
    This example is from \cite{gabbay2021handbook}. Ann and Bob are neighbours, and there is a fence on the boundary between their adjoining properties. Let $p$ denote that a fence is erected. In this example, we can analyse legal relations as follows:
\end{example}
\begin{enumerate}
    \item Ann has a privilege to erect such a fence in the example: $(\oplus_a[a] p\wedge \oplus_a[a]\neg p)\wedge \mathsf{O}_b\neg [b](\neg[a]p\wedge\neg [a]\neg p)$. The first conjunct says that Ann is permitted both erecting a fence and not. The second conjunct expresses that Bob is obliged not to prevent Ann from erecting or not erecting a fence.
    \item Symmetrically, Bob has a privilege to erect such a fence in the example: $(\oplus_b[b] p\wedge \oplus_b[b]\neg p)\wedge \mathsf{O}_a\neg [a](\neg[b]p\wedge\neg [b]\neg p)$.
\end{enumerate}

Now we go back to Example 1 and see how to formalise the mentioned legal relationships. Let $p_a$ mean that the mobile phone is used by Ann, $p_b$ mean that the mobile phone is used by Bob, and $q_a$ means that Ann owns the mobile phone. Then, according to our analysis: 
\begin{enumerate}
    \item Ann has the privilege to use her phone: $(\oplus_a [a]p_a\wedge \oplus_a[a]\neg p_a)\wedge \mathsf{O}_b\neg [b](\neg[a]p_a\wedge \neg[a]\neg p_a)$.
    \item Bob is obliged not to use this mobile phone if Ann does not give permission: $\neg [a]\mathsf{X}\oplus_b [b]p_b\to\mathsf{X}\mathsf{O}_b\neg [b]p_b$. The antecedent says that Ann does not permit Bob using the phone, and the consequent says that Bob ought not to use it.
    \item Ann has the power to extinguish her ownership through abandonment or other acts: $\Diamond[a]\mathsf{U}(q_a,\neg q_a)$. This formula means it is possible that, Ann sees to it that she will not own the phone at some point in the future while keeping her ownership before that.
\end{enumerate}

It should be noticed that we use the propositional letter $q_a$ to express Ann's ownership. Ann's privilege and power, and Bob's obligation mentioned above are all $q_a$'s consequences, so we can write: $q_a\to ((\oplus_a [a]p_a\wedge \oplus_a[a]\neg p_a)\wedge \mathsf{O}_b\neg [b](\neg[a]p_a\wedge \neg[a]\neg p_a))\wedge(\neg [a]\mathsf{X}\oplus_b [b]p_b\to\mathsf{X}\mathsf{O}_b\neg [b]p_b)\wedge\Diamond[a]\mathsf{U}(q_a,\neg q_a)$.

In the next example, we will see how our language works to formalise obligations with time limitation.
\begin{example}
    Bob borrowed a book from Ann at $t_0=0$ and promised to return it no later than $t\in\mathbb{N}^+$. Let $p_a$ and $p_c$ represent that this book is returned to Ann and another individual Carol respectively, and let $q_t$ be a propositional letter only being true at $t$.
\end{example}
\begin{enumerate}
    \item Bob is obliged to return the book to Ann no later than $t$: $\mathsf{O}_b (\mathsf{X}p_a\vee...\vee\underbrace{\mathsf{X...X}}_{t}p_a)$.
    \item Bob is permitted not returning the book before $t$: $\oplus_b [b]\mathsf{U}(\neg p,q_t)$.
    \item Ann has the power to ask Bob to return the book to Carol: $\Diamond[a]\mathsf{O}_b(\mathsf{X}p_c\vee...\vee\underbrace{\mathsf{X...X}}_{t}p_c)$.
\end{enumerate}


Next, we will define $DTS^U$ extended Kripke premodels and $DTS^U$ extended Kripke models, which are used mainly for the completeness proof. 
\begin{definition}
\emph{($DTS^U$ extended Kripke premodel)} A $DTS^U$ extended Kripke premodel is defined as a tuple $\M=(W,R_\Box,\{R_{[i]}\mid i\in Agt\},R_{Agt},\{R_{\mathsf{O}_i}\mid i\in Agt\},R_X,V_U, V)$ where:
\begin{itemize}
    \item $W$ is a nonempty set of possible worlds;
    \item $R_{\Box}$, $R_{[i]}$, $R_{Agt}\subseteq W^2$ are equivalence relations s.t.:
    \begin{enumerate}
        \item[\textbf{(C1)}~~] $R_{[i]}\subseteq R_{\Box}$;
        

        \item[\textbf{(C2)}~~]for all $v, w_i\in W$, where $i\in Agt$, if $w_i \in R_\Box(v)$ for all $i$, then $\bigcap_{i\in Agt} R_{[i]}(w_i)\ne\emptyset$;
    
        \item[\textbf{(C3*)}]for all $ w\in W$, $R_{Agt}(w)\subseteq\bigcap_{i\in Agt} R_{[i]}(w)$;
        
    \end{enumerate}
    \item $R_{X}$ is a relation between worlds in $W$ s.t.:
    \begin{enumerate}
       \item[\textbf{(C4)}~~]$R_X\circ R_\Box\subseteq R_{Agt}\circ R_{X}$. 
    \end{enumerate}
    \item For all $i\in Agt$, $R_{\mathsf{O}_i}\subseteq W^2$ are binary relations satisfying \textbf{(D6)}-\textbf{(D9)}.
\item $V_U: \{\mathsf{U}(\varphi,\psi)\mid \varphi,\psi\in\mathfrak{L}_{DTS^U})\}\to \mathcal{P}(W)$ is a valuation function for all formulas in the form of $\mathsf{U}(\varphi,\psi)$;
 \item $V: P\to \mathcal{P}(W)$ is a valuation function for atomic formulas, where $P$ is the set of propositional letters.
\end{itemize}
\end{definition}

As in $DTS^U$ interpreted systems, $R_\Box(w)$ is the set of worlds that are in the same moments as $w$. $R_X(w)$ is the set of the worlds that are in the next time step of $w$. The Constraint \textbf{(C1)} is the same as \textbf{(D2)}. \textbf{(C2)} corresponds to \textbf{(D4)}, while \textbf{(C3*)} corresponds to \textbf{(D5*)}. \textbf{(C4)} and \textbf{(D3)} express the same requirements. 

Here, I define $V_U$ to simplify the semantics of formulas in the form of $\mathsf{U}(\varphi,\psi)$ and this approach is entirely based on technical considerations. Actually, only in interpreted systems will I define the standard semantics of $\mathsf{U}(\varphi,\psi)$, according to which $\mathsf{U}(\varphi,\psi)$ can be read as "$\varphi$ holds until $\psi$ holds". I will illustrate this point later.


\begin{definition}
{($DTS^U$ extended Kripke model)}\label{superkripke} A $DTS^U$ extended Kripke model is defined as a $DTS^U$ extended Kripke premodel $\M=(W,R_\Box,\{R_{[i]}\mid i\in Agt\},R_{Agt},\{R_{\mathsf{O}_i}\mid i\in Agt\},R_X,V_U,V)$ where $R_X$ is a function.
\end{definition}





\begin{definition}
\emph{(Semantics for $DTS^U$ extended Kripke premodels)} Let $\M=(W,R_\Box,\{R_{[i]}\mid i\in Agt\}, R_{Agt},\{R_{\mathsf{O}_i}\mid i\in Agt\},R_X,V_U,V)$ be a $DTS^U$ extended Kripke premodel. The satisfaction of a formula $\varphi$ in $\mathcal{M}$ is defined accordingly:
\begin{enumerate}
    \item $\M,w \vDash p$ iff $w\in V(p)$;
    \item $\M,w\vDash\neg\varphi$ iff $\M,w \nvDash \varphi$;
    \item $\M,w\vDash\varphi\vee\psi$ iff $\M,w \vDash \varphi$ or $\M,w \vDash \psi$;
    

    \item $\M,w\vDash\Box\varphi$ iff $\forall u\in R_{\Box}(w)$, $\M,u\vDash\varphi$;
    \item $\M,w\vDash[i]\varphi$ iff $\forall u\in R_{[i]}(w)$, $\M,u\vDash\varphi$;
    \item $\M,w\vDash[Agt]\varphi$ iff $\forall u\in R_{Agt}(w)$, $\M,u\vDash\varphi$;
    \item $\M,w\vDash\mathsf{O}_{i}\varphi$ iff $\forall u\in R_{\mathsf{O}_i}(w)$, $\M,u\vDash\varphi$;
    
       
    \item $\M,w\vDash\mathsf{X}\varphi$ iff  $\forall u\in R_X(w),\M,u\vDash\varphi$;

    \item $\M,w\vDash\mathsf{U}(\varphi$,$\psi$) iff  $w\in V_U(\mathsf{U}(\varphi,\psi))$.

\end{enumerate}
\end{definition}

One may be tempted to define the semantics of $\mathsf{U}$ more in line with the meaning of "until", however, we cannot have a proper definition because $R_X$ is not a function, which means we are unable to find a standard semantics of $\mathsf{U} $ as in interpreted systems. Therefore, we only define a simplified semantics of $\mathsf{U}$ and prove that it corresponds to its semantics in interpreted systems (we will do this in the proof of Theorem \ref{29}).





\subsection{Axiomatisation}
In this subsection, I give an axiomatisation w.r.t. the class of $DTS^U$ interpreted systems. I draw inspiration from the axiomatic systems in \cite{van2019neutral}, \cite{halpern2004complete}, \cite{lorini2013temporal},  and \cite{murakami2004utilitarian}.

\begin{definition}\emph{(Axiomatisation of }$\mathsf{DTS}^\mathsf{U}$\emph{)} \label{axiom}
For each $i\in Agt$, we have:

\begin{itemize}
    \item\textbf{(PC)}  All substitution instances of tautologies of classical propositional logic.\\
    
    \item\textbf{(S5$_{\Box}$)}  All S5-principles for the operator $\Box$.\\
    
    \item\textbf{(S5$_{[i]}$)}  All S5-principles for the operators $[i]$.\\
    
     \item\textbf{(S5$_{Agt}$)}  All S5-principles for the operator $Agt$.\\
    
     \item\textbf{(K$_{\mathsf{O}_i}$)}  K-principle for the operator $\mathsf{O}_i$.\\
  
    
    \item\textbf{(}$\Box\to i$\item\textbf{)}  $\Box\varphi\to [i]\varphi$\\

 

   \item\textbf{(}$i\to Agt$\item\textbf{)}   $\bigwedge_{i\in Agt}[i]\varphi_i\to [Agt]\bigwedge_{i\in Agt}\varphi_i$\\

 \item\textbf{(AIA)}  $\bigwedge_{i\in Agt}\Diamond[i]\varphi_i\to \Diamond\bigwedge_{i\in Agt}[i]\varphi_i$\\
 
\item\textbf{(}$\Box\to \mathsf{O}_i$\item\textbf{)}   $\Box\varphi\to \mathsf{O}_i\varphi$\\

\item\textbf{(SE)}   $\oplus_i \top$\\

\item\textbf{(CIC)}   $\mathsf{O}_i\varphi \to \mathsf{O}_i[i]\varphi$\\

\item\textbf{(ID)}  $\mathsf{O}_i\varphi\to\Box\mathsf{O}_i\varphi$ \\
        

        
\item\textbf{(DX)}  $\mathsf{X}\varphi\wedge \mathsf{X}(\varphi\to\psi)\to\mathsf{X}\psi$\\

\item\textbf{(XCom)}  $\mathsf{X}\lnot\varphi\to \neg\mathsf{X}\varphi$\\

\item\textbf{(UInd)}  $\mathsf{U}(\varphi,\psi)\leftrightarrow\psi\vee(\varphi\wedge\mathsf{X}\mathsf{U}(\varphi,\psi))$\\

\item\textbf{(NCUH)}  $[Agt]\mathsf{X}\varphi\to\mathsf{X}\Box\varphi$\\

\item\textbf{(MP)} 
    \begin{tabular}{c}
          $\varphi$, $\varphi\to\psi$ \\
          \hline
         $\psi$
    \end{tabular}\\
   

\item\textbf{(XUInd)} 
\begin{tabular}{c}
$\chi\to\lnot\psi\wedge\mathsf{X}\chi$   \\
\hline
 $\chi\to\lnot\mathsf{U}(\varphi,\psi)$
\end{tabular}\\


\item\textbf{(Necessitation)}  
\begin{tabular}{c}
 $\varphi$   \\
\hline
$\blacksquare\varphi$
\end{tabular},
$\blacksquare\in\{\Box,[Agt],\mathsf{X}\}\cup\{[i]\mid i\in Agt\}\cup\{\mathsf{O}_i\mid i\in Agt\}$.
\end{itemize}

\end{definition}

This axiomatisation includes all tautologies of classical propositional calculus \textbf{(PC)} as well as modus ponens \textbf{(MP)}. Besides, it contains all the principles of the normal modal logic for every operator $\mathsf{O}_i$, and all the principles of the normal modal logic S5 for every operator $[i]$, and $\Box,[A g t]$. Also, we have the rule of necessitation for each modal operator.


\begin{remark}\label{remark}
    According to $(\Box \to i)$, if $\varphi$ happens no matter what every agent does, then every agent sees to it that $\varphi$. In other words, an agent brings about facts that are bound to occur. It is obvious that $(\Box \to i)$ corresponds to \textbf{(D2)} and \textbf{(C1)}. Similarly, $(\Box \to \mathsf{O}_i)$ means that if $\varphi$ happens no matter what every agent does, then every agent ought to see to it that $\varphi$. And it correspondes to \textbf{(D6)}. According to \textbf{$(i \to Agt)$}, all agents bring about together what each of them brings about individually. And \textbf{$(i \to Agt)$} corresponds to \textbf{(D5*)}. \textbf{(AIA)} is an axiom scheme for independence of agents, corresponding to \textbf{(D4)}. \textbf{(SE)} is an axiom scheme for \textbf{(D7)} guaranteeing that $R_{\mathsf{O}_i}$ is serial. \textbf{(CIC)} and \textbf{(ID)} correspond to \textbf{(D8)} and \textbf{(D9)} respectively.

We also have principles for the tense operators. \textbf{(DX)} is the Distribution Axiom for $\mathsf{X}$. \textbf{(XCom)} essentially says that time is deterministic. There is only one way the world can be at the next step, so that if at the next step
$\varphi$ is false, then it is not the case that $\varphi$ can be true at the next step. \textbf{(UInd)} is the interaction axiom between $\mathsf{X}$ and $\mathsf{U}$. Intuitively, it says that $\varphi$ holds until $\psi$
does if and only if either $\psi$ is true now, or $\varphi$ is true now and at the next step it is still the case that $\varphi$ holds until $\psi$ does. Finally, \textbf{(XUInd)} gives us a way to conclude
that $\neg\mathsf{U}(\varphi,\psi)$ holds. 

\textbf{(NCUH)} establishes a fundamental relationship between action and time and corresponds to \textbf{(C4)}: if in the next time step $\varphi$ will be possible then the actual collective choice of all agents will possibly result in a state in which $\varphi$ will be true in the next time step.
\end{remark}


\section{Completeness}
In this section, we prove the weak completeness of the previous axiomatic system w.r.t. $DTS^U$ interpreted systems. The system is only weakly complete, because $\mathsf{DTS^U}$ is not compact. Consider the set $R=\{\mathsf{U}(p,q),p\wedge\neg q,\mathsf{X}(p\wedge\neg q),\mathsf{XX}(p\wedge\neg q),...\}$. This set is finitely satisfiable. This is obvious for a finite $T\subseteq \{p\wedge\neg q,\mathsf{X}(p\wedge\neg q),\mathsf{XX}(p\wedge\neg q),...\}$. For a finite $S\subseteq R$ s.t. $\mathsf{U}(p,q)\in S$, we can always find an $m\in\mathbb{N}$ s.t. for all $n\ge m$, $\underbrace{\mathsf{X}...\mathsf{X}}_n(p\wedge\neg q)\notin S$ and thus we can construct the interpreted system $\mathcal{I}$ in (a) containing a unique history $h$ to satisfy $S$. We can see that since for all $t<n$, $(\mathcal{I},h,t)\vDash p\wedge \neg q$, $(\mathcal{I},h,0)\vDash S\setminus\{\mathsf{U}(p,q)\}$. And since $(\mathcal{I},h,n)\vDash q$, $(\mathcal{I},h,0)\vDash \mathsf{U}(p,q)$.

%\begin{figure}[h]
%    \centering
%\includegraphics[width=0.5\textwidth]{fig/weak completeness.jpg}
%    \caption{Weak Completeness}
%    \label{fig:my_label}
%\end{figure}

Now we consider the whole set $R$. To satisfy $R$ at some point, for example, the starting point, in a history $h'$, $p$ must be true in all possible worlds in $h'$ while $q$ being false in them. As a result, $\mathsf{U}(p,q)$ can never be true at $(h,0)$, rendering the whole $R$ unsatisfiable. You can see this clearly in (b).  

The proof of completeness is divided into 4 steps:

First of all, we concern the completeness of the axiomatic system w.r.t. $DTS^U$ extended Kripke models and construct a canonical model.

Secondly, we make a filtration on the canonical $DTS^U$ extended Kripke model in the style of many-dimensional modal logic to get a premodel. We carry out this operation because our axiomatic system is only weakly complete. We need to first construct a finite Kripke premodel and then transform it into an interpreted system. 

Thirdly, we unravel the extended Kripke premodel after filtration into an interpreted system. It should be noted that, in extended Kripke premodels, we are unable to guarantee that for all $w,v\in W^c$, if $v\in R^c_\Box(w)$, then $v\ne R^c_X(w)$, i.e., there might be $w,v$ s.t. $v$ is in the same moment as $w$, as well as in the future of $w$. This apparently transgresses our intuition about time, but once we unravel the extended Kripke premodel into an interpreted system, such $v$'s are duplicated and fit into different histories. For example, such a $v$ might appear as $(h,t),(h',t'),(h'',t'')...$ in the interpreted system, representing different possible worlds. In this case, since $(h,t)$ and $(h',t')$ are distinct points, $(h,t)$ being in the same moment as some $(h^*,t^*)$ while $(h',t')$ being in the next moment of $(h^*,t^*)$ is no longer a trouble. Besides, after filtration, $R_X$ is no longer a function, rendering time to be indeterministic and  $\textbf{(XCom)}$ does not hold. 
But after unraveling, time will become linear in each history and at each point in the model, there is only a unique point we can reach when going ahead in the course of the current history. Moreover, in interpreted systems, we are able to deal with the operator $\mathsf{U}$ more conveniently and intuitively.

Finally, we show that the set of validities w.r.t. the class of $DTS^U$ interpreted systems is equal to the set of $DTS^U$ super-additive interpreted systems, which means, although our axioms cannot capture all the features of $DTS^U$ interpreted systems, it is still complete w.r.t. them.



\subsection{Canonical $DTS^U$ extended Kripke model}

We prove that the axiomatic system of $\mathsf{DTS^U}$ is complete with respect to the class of $DTS^U$ extended Kripke models. 

\begin{definition}\emph{(Canonical $DTS^U$ extended Kripke model)} The canonical $DTS^U$ extended Kripke model $\M^c$ is the tuple $\M^c=(W^c,R_\Box^c,\{R_{[i]}^c\mid i\in Agt\},R_{Agt}^c,\{R_{\mathsf{O}_i}^c\mid i\in Agt\},R_X^c,V_U^c,V^c)$ where:
\begin{itemize}
    \item $W^c$ is the set of all maximal consistent sets of $DTS^U$ formulas (MCSs);
    \item $R_{\Box}^c, R_{[i]}^c, R_{Agt}^c$, $R_{\mathsf{O}_i}^c$ are respectively the canonical relations for $\Box$, $[i]$, $[Agt]$ and ${\mathsf{O}_i}$, that is: for all $\Gamma, \Delta \in W^c,(\Gamma, \Delta) \in \mathcal{R}_{\blacksquare}^c$ iff for all formulas $\psi, \psi \in \Delta$ implies $\blacklozenge\psi \in \Gamma$, where $\blacksquare\in\{\Box,[Agt]\}\cup\{[i]\mid i\in Agt\}\cup\{\mathsf{O}_i\mid i\in Agt\}$ and $\blacklozenge$ is the dual of $\blacksquare$;
    \item For all $\Gamma, \Delta \in W^c$, $\Delta=R_X^c(\Gamma)$ iff for all formulas $\psi, \psi \in \Delta$ implies $\mathsf{X} \psi \in \Gamma$;
    \item $V^c_U$ is the valuation of formulas in the form of $\mathsf{U}(\varphi,\psi)$ defined by $V^c_U(\mathsf{U}(\varphi,\psi))=\{\Gamma\in W^c\mid \mathsf{U}(\varphi,\psi)\in\Gamma\}$ for all $\mathsf{U}(\varphi,\psi)\in\mathcal{L}_{DTS^U}$;
    \item $V^c$ is the valuation defined by $V^c(p)=\{\Gamma\in W^c\mid p\in\Gamma\}$ for all $p\in P$.
    
\end{itemize}
\end{definition}



\begin{lemma}\emph{(Lindenbaum)}
Let $\varphi$ be a consistent $DTS^U$ formula. There exists an MCS $\Gamma$ s.t. $\varphi\in \Gamma$.
\end{lemma}

\begin{lemma}\emph{(Existence Lemma)}
Let $\Gamma$ be an MCS.
\begin{itemize}
    \item If $\blacklozenge \varphi \in \Gamma$, then there is an MCS $\Delta$ s.t. $(\Gamma, \Delta) \in R_{\blacksquare}^c$ and $\varphi \in \Delta$, where $\blacksquare\in\{\Box,[Agt]\}\cup\{[i]\mid i\in Agt\}\cup\{\mathsf{O}_i\mid i\in Agt\}$ and $\blacklozenge$ is the dual of $\blacksquare$;
    \item If $\mathsf{X} \varphi \in \Gamma$, then there is an MCS $\Delta$ s.t. $R_X^c(\Gamma)= \Delta$ and $\varphi \in \Delta$.
\end{itemize}
\end{lemma}

\begin{lemma}\emph{(Truth Lemma)}\label{truth}
For any MCS $\Gamma$ and for any $DTS^U$ formula $\varphi$, $\M^c, \Gamma \models \varphi$ if and only if $\varphi \in \Gamma$.
\end{lemma}

\begin{lemma}\label{can}
Let $\M^c=(W^c,R_\Box^c,\{R_{[i]}^c\mid i\in Agt\},R_{Agt}^c,\{R_{\mathsf{O}_i}^c\mid i\in Agt\},R_X^c,V^c_U,V^c)$ be the canonical $DTS^U$ extended Kripke model. Then $\M^c$ is a $DTS^U$ extended Kripke model, i.e., $\M^c$ satisfies Definition \ref{superkripke}.
\end{lemma}
\begin{proof}
    Define the canonical general frame $\mathcal{F}=(W^c,R_\Box^c,\{R_{[i]}^c\mid i\in Agt\},R_{Agt}^c,\{R_{\mathsf{O}_i}^c\mid i\in Agt\},R_X^c,\mathcal{A})$, where $\mathcal{A}=\{\{\Gamma\in W^c\mid\varphi\in\Gamma\}\mid\varphi\in\mathcal{L}_{DTS^U}\}$.

For any substitution $\sigma:P\to\mathcal{L}_{DTS^U}$ and valuation $V$, $V_{\sigma}$ is the valuation that maps $p$ to $\{\Gamma\in W^c\mid \sigma(p)\in\Gamma\}\in \mathcal{A}$. We show by induction that for all $\varphi\in\mathcal{L}_{DTS^U}$ in which the operator $\mathsf{U}$ does not appear, $[\varphi]^{\mathcal{F},V_{\sigma}}=[\varphi^\sigma]^{\mathcal{M}^c}$, where $\varphi^\sigma$ is obtained by substituting all propositional letters $p$ in $\varphi$ by $\sigma(p)$.

When $\varphi$ is a propositional letter $p$, $[\varphi]^{\mathcal{F},V_\sigma}=[p]^{\mathcal{F},V_\sigma}=V_\sigma(p)$,
$[\varphi^\sigma]^{\mathcal{M}^c}=[\sigma(p)]^{\mathcal{M}^c}=\{\Gamma\in W^c\mid \sigma(p)\in\Gamma\}$. Therefore, $[\varphi]^{\mathcal{F},V_{\sigma}}=[\varphi^\sigma]^{\mathcal{M}^c}$. Boolean cases are obvious. We consider modal cases. When $\varphi=\Box\psi$, $[\varphi]^{\mathcal{F},V_\sigma}=[\Box\psi]^{\mathcal{F},V_\sigma}=\{\Gamma\in W^c\mid \text{ for all }\Delta\in R^c_\Box(\Gamma), \Delta\in [\psi]^{\mathcal{F},V_\sigma}\}$,
$[\varphi^\sigma]^{\mathcal{M}^c}=[\Box\psi]^{\mathcal{M}^c}=\{\Gamma\in W^c\mid \text{for all }\Delta\in R^c_\Box(\Gamma), \Delta\in [\psi]^{\mathcal{M}^c}\}$. By the inductive hypothesis, $[\psi]^{\mathcal{F},V_{\sigma}}=[\psi^\sigma]^{\mathcal{M}^c}$ and thus $[\varphi]^{\mathcal{F},V_{\sigma}}=[\varphi^\sigma]^{\mathcal{M}^c}$.
The cases when $\varphi=[i]\psi,[Agt]\psi,\mathsf{O}_i\psi,\mathsf{X}\psi$ can be verified similarly.

Since for all $V:P\to\mathcal{A}$, there is a $\sigma$ s.t. $V=V_\sigma$. $\mathcal{F}$ is a descriptive general frame by routine verification. So by Sahlqvist canonicity theorem and the correspondence between our aixoms and properties of $DTS^U$ extended Kripke models illustrated in Remark \ref{remark}, $\M^c$ is a $DTS^U$ extended Kripke model.
\end{proof}





We have to mention that $R_X^c$ is exactly a function since $\M^c\vDash$\textbf{(XCom)}. But after we make a filtration on $\M^c$ in Subsection 3.2, the resulting $R^f_X$ might not be a function. As we will see in Subsection 3.2, the obtained model is not necessarily a $DTS^U$ extended Kripke model but a $DTS^U$ extended Kripke premdel.


\subsection{Filtration in the style of many-dimensional modal logic}

In this subsection, we show how to make a filtration on the canonical model obtained in the previous subsection in the style of many-dimensional modal logic \cite{gabbay2003many}. In this proof, we treat $R_\Box$ as the most fundamental relation and define a new equivalence relation $\sim$ based on it, according to which we partition the original set of possible worlds $W$ to get a new set of possible worlds. We will first define $\sim$, then define $R^f_{\Box}, R^f_{[i]},R^f_{Agt},R^f_{\mathsf{O}_i}, R^f_X$.

\begin{definition}
    Let $\mathcal{M} = (W,R_\Box,\{R_{[i]}\mid i\in Agt\},R_{Agt},\{R_{\mathsf{O}_i}\mid i\in Agt\},R_X,V_U,V)$ be a model  satisfying Definition \ref{superkripke}. $\Sigma$ is an arbitrary finite set of $DTS^U$ formulas closed under subformulas, and satisfying the condition that: (1) for all $\mathsf{U}(\varphi_1,\varphi_2)\in\Sigma$, $\mathsf{XU}(\varphi_1,\varphi_2)\in\Sigma$; (2) for all $\mathsf{O}_i\varphi\in\Sigma$, $[i]\varphi\in\Sigma$. Then the filtration $\M^f=(W^f,R_\Box^f,\{R_{[i]}^f\mid i\in Agt\},R_{Agt}^f,\{R_{\mathsf{O}_i}^f\mid i\in Agt\},R_X^f,V_U^f,V^f)$ of $\M$ through $\Sigma$ is defined as follows:
    \begin{itemize}
        \item For any $w \in W$, let $\Sigma(w) = \{\varphi \in \Sigma \mid \mathcal{M}, w \models \varphi\}$. For any $w, v \in W$, $w \sim v$ iff 
\[
    \Sigma(w) = \Sigma(v) \text{ and } \{\Sigma(x) \mid w R_\Box x\} = \{\Sigma(x) \mid v R_\Box x\}
\]
$|w| = \{x \in W \mid x \sim w\}$
\item $|w|R^f_\blacksquare|v|$ iff $\exists w' \in |w|\exists v' \in |v|, w'R_\blacksquare v'$, where $\blacksquare\in\{\Box,[Agt],\mathsf{X}\}$;
\item For all $i\in Agt$, 
\begin{itemize}
    \item $|w|R^p_{[i]}|v|$ iff $\exists w' \in |w|\exists v' \in |v|, w'R_{[i]} v'$.
    \item $R^f_{[i]}$ is the transitive closure of $R^p_{[i]}$.  
    
\end{itemize}

\item For all $i\in Agt$, 
\begin{itemize}
    \item $|w|R^p_{\mathsf{O}_i}|v|$ iff $\exists w' \in |w|\exists v' \in |v|, w' R_{\mathsf{O}_i}v'$.
    \item $R^f_{\mathsf{O}_i}=R^p_{\mathsf{O}_i}\circ R_{[i]}^f$.
\end{itemize}
\item $V^f(p)=\{|w|\mid \mathcal{M},w\vDash p\}$ for all propositional letters $p\in\Sigma$;
\item $V^f_U(\mathsf{U}(\varphi,\psi))=\{|w|\mid \M,w\vDash\mathsf{U}(\varphi,\psi)\}$ for all $\mathsf{U}(\varphi,\psi)\in\Sigma$.
\end{itemize}
\end{definition}

\begin{lemma}\label{sim}
$\sim$ is an equivalence relation. 
\end{lemma}
\begin{proof}
Reflexivity and symmetry follows from the definition of $\sim$. We only need to illustrate the transitivity of $\sim$. Suppose that $x\sim y\sim z$, then $\Sigma(x)=\Sigma(y)=\Sigma(z)$, $\{\Sigma(w)\mid x R_\Box w\}=\{\Sigma(w)\mid y R_\Box w\}=\{\Sigma(w)\mid z R_\Box w\}$. Therefore, $x\sim z$.
\end{proof}

The following lemma claims that $\sim$ and $R_{\Box}$ commute. 

\begin{lemma}\label{commute}
   $\exists y, x \sim y R_\Box z$ iff  $\exists z', x R_\Box z' \sim z$. 
\end{lemma}
\begin{proof}
It is enough to show only one direction, since the other follows by 
taking the converse and using the fact that both $\sim$ and $R_\Box$ are symmetric. 
Suppose $x \sim y R_\Box z$. By the definition of $\sim$, there exists a $z'$ s.t. 
$xR_\Box z'$ and $\Sigma(z')=\Sigma(y)$. We claim that $z'\sim z$ holds. Since $R_\Box$ is an equivalence relation,  
$\{w \mid xR_\Box w\} = \{w \mid z'R_\Box w\}$ and $\{w \mid zR_\Box w\} = \{w \mid yR_\Box w\}$. From $x\sim y$, we infer that $\{\Sigma(w)\mid xR_\Box w\}=\{\Sigma(w)\mid yR_\Box w\}$. Therefore, $\{\Sigma(w) \mid zR_\Box w\} = \{\Sigma(w) \mid z'R_\Box w\}$. Then by the definition of $\sim$, $z'\sim z$.

 
\end{proof}


Proposition \ref{1}-\ref{2} demonstrate that $\M^f$ satisfies the requirements of a $DTS^U$ extended Kripke premodel. 


\begin{proposition}\label{1}
    $R^f_\Box$ is an equivalence relation. 
\end{proposition}
\begin{proof}
   The reflexivity and symmetry of $R^f_\Box$ can be seen easily. We only show that $R^f_\Box$ is transitive. Suppose $|x|R^f_\Box|y|R^f_\Box|z|$. Then there are $x',y',y'',z'\in W$ s.t. $x\sim x'R_\Box y'\sim y \sim y''R_\Box z'\sim z$. Thus, $x'R_\Box y'\sim y''$. Since $R_\Box$ and $\sim$ commute, there is an $x''$ s.t. $x\sim x'' R_\Box y''$. By the transitivity of $R_\Box$, $x\sim x''R_\Box z'\sim z'$. As a result, $|x|R^f_\Box |z|$.
\end{proof}



\begin{proposition}
For all $\blacksquare\in\{[Agt]\}\cup\{[i]\mid i\in Agt\}$, $R_{\blacksquare}^f$ is an equivalence relation.
\end{proposition}


\begin{proposition}\label{22}
$R_{\Box}^f$, every $R_{[i]}^f$, $R_{Agt}^f$ satisfy \textbf{(C1),(C2)} and \textbf{(C3*)}.
\end{proposition}
\begin{proof}
First, we show that $R_{\Box}^f$ and every $R_{[i]}^f$ satisfy \textbf{(C1)}. Assume that for $|w|,|v|\in W^f$, $|w|R_{[i]}^f|v|$. Then there are $w'\in|w|,v'\in|v|$ s.t. $w\sim w'R_{[i]}v'\sim v$. Since $R_{[i]}\subseteq R_{\Box}$, $w\sim w'R_{\Box}v'\sim v$, then $|w|R_{[i]}^f|v|$. 

Next, we show that $R_{\Box}^f$ and every $R^f_{[i]}$ satisfy \textbf{(C2)}. Assume that for $|v|, |w_1|,...,|w_n|\in W^f$, $|w_i|  R_\Box^f|v|$ for all $i$. Then there are $w_1'\in|w_1|,...,w_n'\in |w_n|, v_1,...,v_n\in |v|$ s.t. $w_i' R_\Box v_i\sim v$ for all $i$. By Lemma \ref{commute}, there is a $w_i''\in|w_i|$ s.t. $w_i'\sim w_i'' R_\Box v$. Since $\bigcap_{i\in Agt} R_{[i]}(w_i'')\ne\emptyset$, pick a $w\in\bigcap_{i\in Agt} R_{[i]}(w_i'')$, $|w|\in\bigcap_{i\in Agt} R_{[i]}^f(|w_i|)\ne\emptyset$.


Finally, we prove that $R_{Agt}^f$ and every $R_{[i]}^f$ satisfy \textbf{(C3*)}. Assume that for $|w|,|v|\in W^f$, $|w|R_{Agt}^f|v|$. Then there are $w'\in|w|,v'\in|v|$ s.t. $w'R_{Agt}v'$. As a result, $w'R_{[i]}v'$ for all $i\in Agt$. Further,  $|w|R_{[i]}^f|v|$ for all $i\in Agt$. Therefore, $|v|\in\bigcap_{i\in Agt} R_{[i]}^f(|w|)$.
\end{proof}

\begin{proposition}\label{33}
$R_{\Box}^f$, $R_X^f$ and $R^f_{Agt}$ satisfy  \textbf{(C4)}.
\end{proposition}
\begin{proof}
We need to show: if $|x|R^f_X|y|R^f_\Box|z|$ then $\exists u, |x|R^f_{Agt}|u|R_X^f|z|$. 
Suppose $|x|R^f_X|y|R^f_\Box|z|$, then there are $x' \in |x|, y' ,y'' \in |y|, z' \in |z|$ s.t. $x'R_Xy'\sim y''R_\Box z'$. Since $R_\Box$ and $\sim$ compute, we find $z''$ s.t. $y' R_\Box z'' \sim z'$. So $x' R_X y' R_\Box z''$ in the original model. By \textbf{(C4)} there is a $u$ s.t. $x' R_{Agt} u R_X z''$. 
\end{proof}

\begin{proposition}\label{2}
$R_{\Box}^f$, every $R_{\mathsf{O}_i}^f$, $R_{[i]}^f$ satisfy \textbf{(D6)}-\textbf{(D9)}.
\end{proposition}
\begin{proof}
We can prove that $R_{\mathsf{O}_i}^f$ satisfies {\textbf{(D6)}} in the similar way we prove $R_{[i]}^f$ satisfies {\textbf{(C1)}}.
        
Then we show that every $R_{\mathsf{O}_i}^f$ satisfies {\textbf{(D7)}}. For an arbitrary $|w|\in W^f$, by \textbf{(D7)}, there exists a $v\in W$ s.t. $wR_{\mathsf{O}_i} v$. Therefore, there exists a $|v|\in W^f$ s.t. $|w|R_{\mathsf{O}_i}^f |v|$. 

Next, we should prove that every $R_{\mathsf{O}_i}^f$,  $R^f_{[i]}$ satisfy \textbf{(D8)}. Suppose there are $|w|,|v|,|u|\in W^f$ s.t. $|w| R_{\mathsf{O}_i}^f|v|R_{[i]}^f|u|$, By the definition of $R^f_{\mathsf{O}_i}$, there is a $|v'|\in W^f$ s.t. $|w| R_{\mathsf{O}_i}^p|v'|R_{[i]}^f|v|R_{[i]}^f|u|$, so $|w| R_{\mathsf{O}_i}^p|v'|R_{[i]}^f|u|$, and then $|w| R_{\mathsf{O}_i}^f|u|$.

Finally, we verify that $R_{\Box}^f$ and every $R_{\mathsf{O}_i}$ satisfy \textbf{(D9)}. Suppose $|w|,|v|,|u|\in W^f$ and $|w|R_{\Box}^f|v|R_{\mathsf{O}_i}^f|u|$. Then we can find $w'\in |w|$ , $v',v''\in|v|$, $u'\in|u|$, s.t. $w'R_{\Box}v'\sim v\sim v
''R_{\mathsf{O}_i}u'$. Since $\sim$ and $R_\Box$ commute, there is a $w''\in W$ s. t. $w'\sim w'' R_\Box v\sim v' R_{\mathsf{O}_i}u'$. Again, we find an $w'''$ s.t. $w'\sim w''\sim w''' R_\Box v' R_{\mathsf{O}_i}u'$. By \textbf{(D9)}, $ w''' R_{\mathsf{O}_i}u'$. Therefore, $ |w| R_{\mathsf{O}_i}^f|u|$.
\end{proof}

We need the following lemma in the proof of Theorem \ref{filtration thm}, so we list it separately.

\begin{lemma}\label{lemma7}
For any $[i]\varphi \in \Sigma$, for any $w, v \in W$ s.t. $|w| R^f_{[i]} |v|$, if $\mathcal{M}, v \not\models \varphi$ then $\mathcal{M}, w \not\models [i]\varphi$. 
\end{lemma}

\begin{theorem}{(Filtration Theorem)}\label{filtration thm}
For all $\varphi\in\Sigma$, for all $w\in W$, $\M,w\vDash\varphi$ iff $\M^f,|w|\vDash\varphi$.
\end{theorem}
\begin{proof}
We show this by induction on $\varphi$. The base case is immediate from the definition of $V^f$.
The boolean cases are straightforward, for the fact that $\Sigma$ is closed under subformulas
allows us to apply the inductive hypothesis.

Now we consider modal cases.

Firstly, suppose $\Diamond \varphi \in \Sigma$ and $\M, w \vDash \Diamond \varphi$. Then there is a $v$ s.t. $wR_{\Box} v$ and $\M, v \vDash \varphi$. By the definition of $R_{\Box}^f$, $|w|R_{\Box}^f|v|$. As $\Sigma$ is subformula closed, $\varphi \in \Sigma$. Thus, by the inductive hypothesis $\M^f,|v| \vDash \varphi$. Hence, $\M^f,|w| \vDash \Diamond \varphi$.
Conversely, suppose $\Diamond \varphi \in \Sigma$ and $\M^f,|w| \vDash \Diamond \varphi$. Thus, there is a state $|v|$ in $\M^f$ s.t. $|w|R_{\Box}^f|v|$ and $\M^f,|v| \vDash \varphi$. As $\varphi \in \Sigma$, by the inductive hypothesis $\M, v \vDash \varphi$. So there are $w',v'$ s.t. $w\sim w'R_{\Box}v'\sim v$. Since $\varphi\in \Sigma$, $\M, v' \vDash \varphi$. Hence, $\M, w' \vDash \Diamond\varphi$. By $\Diamond\varphi\in \Sigma$, we conclude that $\M, w \vDash \Diamond \varphi$. 

Similarly, we can prove the case of $\langle Agt\rangle\varphi$ and $\neg\mathsf{X}\neg\varphi$.

Secondly, suppose for some $i\in Agt$, $\langle 
 i\rangle \varphi \in \Sigma$ and $\M, w \vDash \langle i\rangle\varphi$. Then $\M^f,|w| \vDash \langle i\rangle\varphi$. Conversely, suppose $\langle i\rangle \varphi \in \Sigma$ and $\M^f,|w| \vDash \langle i\rangle \varphi$. Thus, there is a state $|v|$ in $\M^f$ s.t. $|w|R_{[i]}^f|v|$ and $\M^f,|v| \vDash \varphi$. As $\varphi \in \Sigma$, by the inductive hypothesis $\M, v \vDash \varphi$. By the definition of $R^f_{[i]}$, $|w|(R^p_{[i]})^n|v|$, $n\in\{1,2,...\}$. We proceed by induction to show that for all $n\in\{1,2,...\}$, $\M,w\vDash\langle i\rangle\varphi$.

 When $n=1$, there are $w',v'$ s.t. $w\sim w'R_{[i]}v'\sim v$. Since $\varphi\in \Sigma$, $\M, v' \vDash \varphi$. Hence, $\M, w' \vDash \langle i\rangle\varphi$, $\M, w \vDash \langle i\rangle\varphi$. When $n=k+1$ for some $k\ge 0$, there is a $|u|$ s.t.  $|w|R^p_{[i]}|u|(R^p_{[i]})^k|v|$. By the inductive hypothesis, $\M, u \vDash \langle i\rangle\varphi$. Hence, there are $w',u'$ s.t. $w\sim w'R_{[i]}u'\sim u$. So $\M, u' \vDash \langle i\rangle\varphi$, $\M, w' \vDash \langle i\rangle\langle i\rangle\varphi$. By the transitivity of $R_{[i]}$, $\M, w' \vDash \langle i\rangle\varphi$. Therefore, we conclude that $\M, w \vDash \langle i\rangle\varphi$. 


Thirdly, we need to show, for any $\mathsf{O}_i\varphi \in \Sigma$, for any $w \in W$, $\mathcal{M}, w \models \mathsf{O}_i\varphi$ iff $\mathcal{M}, |w| \models \mathsf{O}_i \varphi$. We only show the left-to-right direction. Suppose $\mathcal{M}^f, |w| \not\models \mathsf{O}_i\varphi$. Then there is a $|v| \in W^f$ s.t. $|w| R_{\mathsf{O}_i}^f |v|$ and $\mathcal{M}^f, |v| \not\models \varphi$. 
Then there is a $|u|\in M^f$ s.t. $|w| R^p_{\mathsf{O}_i} |u| R^f_{[i]} |v|$. By the inductive hypothesis, $\mathcal{M}, v \not\models\varphi$. By the closure property of $\Sigma$, $[i]\varphi \in \Sigma$. By Lemma \ref{lemma7}, $\mathcal{M}, u \not\models [i]\varphi$. Since $|w| R^p_{\mathsf{O}_i} |u|$, there are $w'\in|w|$, $u' \in |u|$ s.t. $w' R_{\mathsf{O}_i}u'$. Also, $\mathcal{M}, u' \not\models [i]\varphi$. Then $\mathcal{M}, w' \not\models \mathsf{O}_i[i]\varphi$. By \textbf{(CIC)} $\mathcal{M}, w' \not\models \mathsf{O}_i\varphi$. Therefore, $\mathcal{M}, w \not\models \mathsf{O}_i\varphi$.

At last, we should consider formulas in the form of $\mathsf{U}(\varphi,\psi)$. It is obvious that $\mathcal{M}^f,|w|\vDash\mathsf{U}(\varphi,\psi)$ iff $\M,w\vDash\mathsf{U}(\varphi,\psi)$ by our definition of $V^f_U$.
\end{proof}

\subsection{Unraveling to an interpreted system}
In this subsection, we unravel the model obtained in Subsection 3.2 to an interpreted system. So far, we have only concerned the simplified semantics of $\mathsf{U}$, now it is time to take the standard semantics of $\mathsf{U}$ into consideration. Before unraveling, we firstly show that, after filtration, formulas in the form of $\mathsf{U}(\varphi_1,\varphi_2)$ in $\Sigma$ can be satisfied if we read them as "$\varphi_1$ holds until $\varphi_2$ holds". The methods used in this subsection is inspired by \cite{halpern2004complete}.

For each $|w|\in W^f$, let $\varphi_w=\bigwedge\{\varphi\in\Sigma\mid\M^f,|w|\vDash\varphi\}$. For each $T\subseteq W^f$, let $\varphi_T=\bigwedge\{\varphi\in\Sigma\mid\M^f,|w|\vDash\varphi\text{ for all }|w|\in T\}$.



\begin{lemma}\label{24}
For all formulas $\varphi, \psi$ and $\chi$, if $\vdash \varphi \to \neg \chi$ and $\vdash \varphi \to \mathsf{X}(\varphi \vee(\neg \psi \wedge \neg \chi))$ then $\vdash \varphi \to \neg(\mathsf{U}(\psi, \chi))$
\end{lemma}
\begin{proof}
Suppose that $\vdash \varphi \to \neg\chi\wedge\mathsf{X}(\varphi \vee(\neg \psi \wedge \neg \chi))$. By the left-to-right \textbf{(UInd)}, $\vdash\mathsf{U}(\psi,\chi)\to\chi\vee(\psi\wedge\mathsf{XU}(\psi,\chi))$. So we can obtain that $\vdash \varphi \wedge\mathsf{U}(\psi , \chi) \to\neg \chi \wedge \mathsf{X}\mathsf{U}(\psi , \chi) \wedge \mathsf{X}(\varphi \vee(\neg \psi \wedge \neg \chi))$. Then, by the left-to-right \textbf{(UInd)} again, $\vdash\mathsf{U}( \psi,  \chi) \to ( \psi \vee  \chi)$. Hence, $\vdash\mathsf{X}\mathsf{U}( \psi,  \chi) \to \mathsf{X}( \psi \vee  \chi)$ by the necessitation rule for $\mathsf{X}$. Also, it is easy to notice that $\vdash\mathsf{X}(\varphi\vee(\neg\psi\wedge\neg\chi))\leftrightarrow\mathsf{X}((\psi\vee\chi)\to\varphi)$. Thus, it follows using \textbf{(DX)} that $\vdash\mathsf{X}\mathsf{U}(\psi , \chi) \wedge \mathsf{X}(\varphi \vee(\neg \psi \wedge \neg \chi))\to \mathsf{X}\varphi$. Therefore, $\vdash\varphi\wedge\mathsf{U}(\psi,\chi)\to\neg\chi\wedge\mathsf{X}\varphi$ and thus $\vdash \varphi \wedge\mathsf{U}(\psi,  \chi) \to \neg \chi \wedge \mathsf{X}(\varphi \wedge\mathsf{U}(\psi , \chi))$. Now using \textbf{(XUInd)} we obtain $\vdash \varphi \wedge\mathsf{U}(\psi, \chi) \to \neg\mathsf{U}(\psi, \chi) $, which implies that $\vdash \varphi \to \neg\mathsf{U}(\psi , \chi)$.
\end{proof}


\begin{lemma}\label{26}
If $\mathsf{U}(\varphi_1 , \varphi_2) \in \Sigma$, then $\M^f,|w| \vDash\mathsf{U}(\varphi_1 , \varphi_2)$ iff there exists a sequence $|w|=|w_0|,|w_1|,\ldots ,\\|w_n|$, s.t. for all $k\in\{0,1,...,n-1\}$, $|w_{k+1}|\in R_X^f(|w_k|)$, s.t. $\M^f,|w_n| \vDash\varphi_2$, and $\M^f,|w_k| \vDash\varphi_1$ for all $k<n$.
\end{lemma}
\begin{proof}
Note that if $\mathsf{U}(\varphi_1 , \varphi_2)$ is in $\Sigma$, then $\varphi_1, \varphi_2\in\Sigma$. We first show the right-to-left direction. 

  We proceed by induction on $n$. When $n=0$, $\M,w_0\vDash{\varphi_2}$, by \textbf{(UInd)}, $\M,w_0\vDash{\mathsf{U}(\varphi_1,\varphi_2)}$. When $n=m+1$, we know that $|w_0|,|w_1|,|w_2|,\ldots ,|w_{m+1}|$ is a sequence s.t. for all $k\in\{1,2,...,m\}$, $|w_{k+1}|\in R_X^f(|w_k|)$, then according to the inductive hypothesis, $\M^f,|w_1|\vDash \mathsf{U}(\varphi_1 , \varphi_2) $. Since $|w_{1}|\in R_X^f(|w_0|)$ and $\mathsf{XU}(\varphi_1,\varphi_2)\in\Sigma$ by the definition of $\Sigma$, $\M^f,|w_0|\vDash \mathsf{X}\mathsf{U}(\varphi_1 , \varphi_2)$. By assumption, we also have $\M^f,|w_0|\vDash\varphi_1$. Therefore, $\M,w_0\vDash \mathsf{X}\mathsf{U}(\varphi_1 , \varphi_2)\wedge\varphi_1$. Then by \textbf{(UInd)}, $\M,w_0\vDash\mathsf{U}(\varphi_1 , \varphi_2)$. Hence, $\M^f,|w_0|\vDash\mathsf{U}(\varphi_1 , \varphi_2)$.

Then we show the other direction.
Suppose towards a contradiction that $\mathcal{M}^f,|w|\vDash \mathsf{U}(\varphi_1 , \varphi_2)$ and no appropriate sequence exists. We then have $\mathcal{M},w\vDash \mathsf{U}(\varphi_1 , \varphi_2)$. By \textbf{(UInd)}, $\mathcal{M},w\vDash (\varphi_1\wedge\mathsf{XU}(\varphi_1 , \varphi_2))\vee\varphi_2$. Therefore,  $\mathcal{M},w\vDash \varphi_1\vee\varphi_2$. If $\mathcal{M},w\vDash\varphi_2$, then $|w|$ is an appropriate sequence and thus $\mathcal{M},w\vDash\varphi_1$.


Let $T\subseteq W^f$ be the smallest set of states s.t.: (i) $|w|\in T$; (ii) if $|v| \in T$, $|u|\in R^f_X(|v|)$, and $\mathcal{M}^f,|u|\vDash\varphi_1$, then $|u| \in T$. Then, for all $|t|\in T$, there is an $m\in\mathbb{N}$ s.t. $|t|\in (R^f_X)^m(|w|)$. We proceed an induction on $m$ to show that:  $\M^f,|t|\vDash\neg\varphi_2$. 
When $m=0$, which means $|t|=|w|$, if $\M^f,|t|\vDash\varphi_2$, then $|w|$ is an appropriate sequence. This contradicts our assumption. When $m=k+1$, by the inductive hypothesis, for all $|v'|\in T$ which can be reached in at most $k$ $R^f_X$-steps from $|w|$,  $\M^f,|v'|\vDash\neg\varphi_2$. Moreover, when $|v'|\ne|t|$, $\mathcal{M}^f,|v'|\vDash\varphi_1$. If $\M^f,|t|\vDash\varphi_2$, then $|w|,...,|t|$ is an appropriate sequence.
Therefore, $\M^f,|t|\vDash\neg \varphi_2$ for all $|t| \in T$, so $\vdash \varphi_T \to\neg \varphi_2$. 

In addition, for each $|t| \in T$ and  $|u|$ s.t. $|u|\in R^f_X(|t|)$, we have either $|u| \in T$ or $\M^f,|u|\vDash\neg \varphi_1 \wedge \neg \varphi_2$. This is because, if $\M^f,|u|\vDash \varphi_1$, then $|u|\in T$. If $\M^f,|u|\vDash \varphi_2$, then $|u|$ and the elements in $T$ that are able to reach $|t|$ through $R^f_X$ can together form an appropriate sequence.
Thus, we obtain $\vdash \varphi_T \to \mathsf{X}(\varphi_T \vee(\neg \varphi_1 \wedge \neg \varphi_2))$. It now follows using Lemma \ref{24} that $\vdash \varphi_T \to \neg\mathsf{U}(\varphi_1 , \varphi_2)$. In particular, since $|w| \in T$, we have $|w|\vDash\neg\mathsf{U}(\varphi_1 , \varphi_2)$, which contradicts the assumption that $\mathcal{M}^f,|w|\vDash \mathsf{U}(\varphi_1 , \varphi_2)$.
\end{proof}

From now on, we sometimes use $\rightarrow$ to replace $R_X^f$ for convenience, and substitute expressions in the form of $|u|\in R^f_X(|v|)$ with $|v|\rightarrow|u|$.
We say that a $\rightarrow$-sequence of states $|w_0|,| w_1|, \ldots$, is \textit{acceptable} if for all $n \geq 0$, $\mathsf{U}(\varphi_1,\varphi_2)\in\Sigma$, if $|w_n|\vDash\mathsf{U}(\varphi_1 ,\varphi_2)$ then there exist $m,n$ s.t. $m\ge n$ and $|w_m| \vDash\varphi_2$ and $|w_k| \vDash \varphi_1$ for all $k$ with $n \le k<m$.

\begin{lemma}\label{266}
Every finite $\rightarrow$-sequence of states in $\M^f$ can be extended to an infinite acceptable sequence.
\end{lemma}
\begin{proof}
To see this, first note that for every $|w|$ there exists a state $|v|$ with $\varphi_w\wedge \mathsf{X}\varphi_v$ consistent. Because $\vdash  \bigvee_{|v|\in W^f}\varphi_v$, and by \textbf{(Nessecitation)} of $\mathsf{X}$,  $\vdash \mathsf{X} \bigvee_{|v|\in W^f}$  $\varphi_v$. Thus, every finite sequence of states can be extended to an infinite sequence, and it remains to show that the obligations arising from the until formulas can be satisfied.

Suppose the finite $\rightarrow$-sequence is $|w_0| \rightarrow \ldots \rightarrow |w_n|$. Now, for any formula $\mathsf{U}(\varphi_1 , \varphi_2) $ s.t. $\M^f, |w_0|\vDash\mathsf{U}(\varphi_1 , \varphi_2)$, it follows from the definition of $V_U^f$ that  $\M, w_0\vDash\mathsf{U}(\varphi_1 , \varphi_2)$. Note that \textbf{(UInd)} might not hold in $\M^f$, so we have to step back and use \textbf{(UInd)} only in $\M$. By \textbf{(UInd)}, either $\M, w_0\vDash\varphi_2$, or else $\M, w_0\vDash\varphi_1\wedge\mathsf{XU}(\varphi_1 , \varphi_2)$. In the first case, $\M^f, |w_0|\vDash\varphi_2$. In the latter case, $\M^f, |w_0|\vDash\varphi_1$ and  $\M^f, |w_1|\vDash\mathsf{U}(\varphi_1,\varphi_2)$. So $\M, w_1\vDash\mathsf{U}(\varphi_1 , \varphi_2)$. Again by \textbf{(UInd)}, either $\M, w_1\vDash\varphi_2$, or else $\M, w_1\vDash\varphi_1\wedge\mathsf{XU}(\varphi_1 , \varphi_2)$. Thus, either $\M^f, |w_1|\vDash\varphi_2$ or $\M^f, |w_1|\vDash\varphi_1$ and $\M, w_2\vDash\mathsf{U}(\varphi_1 , \varphi_2)$... By repeating this procedure, we can conclude that, either $\M^f,|w_k|\vDash{\varphi_2}$ for some $k\in\{0,...,n\}$, and $\M^f,|w_m|\vDash\varphi_1$ for all $m\in\{0,...,k-1\}$, or else $\M^f,|w_n|\vDash{\mathsf{U}(\varphi_1,\varphi_2)}$ and $\M^f, |w_m|\vDash\varphi_1$ for all $m\in\{0,...,n-1\}$. In the latter case, by Lemma \ref{26}, there exists a sequence $|w_n| \rightarrow |w_{n+1}| \rightarrow \ldots \rightarrow |w_{n^{\prime}}|$ s.t. $|w_{n^{\prime}}|\vDash\varphi_2$ and $|w_m|\vDash\varphi_1$ for $m\in\{n,\ldots,n^{\prime}-1\}$.This gives a finite extension of the original sequence that satisfies the obligation imposed by $\mathsf{U}(\varphi_1, \varphi_2)$ at $|w_0|$. Applying this argument to the remaining obligations at $|w_0|$, we eventually obtain a sequence that satisfies all the obligations at $|w_0|$. We may then move on to $|w_1|$ and apply the same procedure. It is clear that we can obtain an acceptable sequence extending the original sequence.
\end{proof}


Notationally, when $h$ is a sequence of states, $h_i$ is the $i$-th element of $h$. 
Now we unravel $\M^f$ into $\mathcal{I}=(H, R_\Box^s, \{R_{[i]}^s\mid i\in Agt\}, R_{Agt}^s,\{R_{\mathsf{O}_i}^s\mid i\in Agt\}, V^s)$:
\begin{itemize}
    \item $H\subseteq (W^f)^\omega$ is the set of all infinite acceptable sequence of $\mathcal{M}^f$;
    \item $(h, t) R_{Agt} ^s (h', u)$ iff $t= u$ and $h_{t'} R^f_{Agt} h'_{t'}$ for all $t'\le t$ in $\mathcal{M}^f$;
    \item $(h, t) R_\Box ^s (h', u)$ iff $t= u$, $h_t R_\Box^f h'_u$ and $(h,t') R^s_{Agt} (h',t')$ for all $t'< t$;
    \item $(h, t) R_\blacksquare ^s (h', u)$ iff $(h, t) R_\Box ^s (h', u)$ and $h_t R^f_{\blacksquare} h'_u$ in $\mathcal{M}^f$, where $\blacksquare\in\{[i]\mid i\in Agt\}\cup\{\mathsf{O}_i\mid i\in Agt\}$;
    \item $(h, t) \in V^s(p)$ iff $h_t \in V^f(p)$.
\end{itemize}

Note that we place special requirements on $R_\Box^s$ because we want $\mathcal{I}$ to satisfy \textbf{(D3)}. Although $\M^f$ satisfies \textbf{(C4)} and \textbf{(C4)} corresponds to \textbf{(D3)}, $\mathcal{I}$ would lose this property if we simply unravel $\M^f$ without defining $R^s_\Box$ with additional rules.

\begin{lemma}\label{263}
    For all $x,y\in W^f$, $x R^f_X y$ iff there exist $h\in H$ and $t\in\mathbb{N}$ s.t. $x=h_t$, $y=h_{t+1}$.
\end{lemma}
\begin{proof}
The left-to-right direction follows from Lemma \ref{266}, and the right-to-left direction follows from the definition of acceptable sequences.
\end{proof}

\begin{lemma}\label{122}
    $\mathcal{I}$ is a $DTS^U$ super-additive interpreted system.
\end{lemma}
\begin{proof}
Firstly, $R_{Agt}^s$ is an equivalence relation. We only show transitivity. Assume that $(h,t)R_{Agt}^s(h',t)\\ R_{Agt}^s(h'',t)$. Then $h_{t'}R_{Agt}^f h_{t'}'R_{Agt}^f h_{t'}''$ for all $t'\le t$. By the transitivity of $R_{Agt}$, $h_{t'}R_{Agt} h_{t'}''$ for all $t'\le t$, so $(h,t)R_{Agt}^s(h'',t)$.

Secondly, we show $R_\Box^s$ is an equivalence relation. Reflexivity is easy. We show symmetry and transitivity. Assume that $(h,t)R_\Box^s(h',t)R_\Box^s(h'',t)$. Then $h_tR_\Box^f h_t'R_\Box^f h_t''$, and $(h,t')R_{Agt}^s(h',t')R_{Agt}^s(h'',t')$ for all $t'<t$. Since $R_\Box^f$ is an equivalence relation, we have $h_tR_\Box^f h_t''$ and $h_t'R_\Box^f h_t$. Also, since $R_{Agt}^s$ is an equivalence relation, $(h,t')R_{Agt}^s(h'',t')$ and $(h',t')R_{Agt}^s(h,t')$ for all $t'<t$. Therefore, $(h,t)R_\Box^s(h'',t)$ and $(h',t)R_\Box^s(h,t)$.

$R_{[i]}^s$ is an equivalence relation because $R_{[i]}$ and $R_{\Box}^s$ are equivalence relations.
 $\mathcal{I}$ satisfies \textbf{(D1)}-\textbf{(D3)} and \textbf{(D6)} by definition. And $\mathcal{I}$ satisfies \textbf{(D4)}, \textbf{(D7)}-\textbf{(D9)} because $R_\Box^s$ is transitive and $\mathcal{M}^f$ satisfies \textbf{(D7)}-\textbf{(D9)}. We show $\mathcal{I}$ satisfies \textbf{(D8)} as an example. Assum that $(h,t)R_{\mathsf{O}_i}^s(h',t)$ and $(h',t)R_{[i]}^s(h'',t)$. By the definition of $R_{\mathsf{O}_i}^s$ and $R_{[i]}^s$, $h_tR_{\mathsf{O}_i}^f h'_t$, $h'_tR_{[i]}^f h''_t$, and $(h,t)R_{\Box}^s(h',t)R_{\Box}^s(h'',t)$. Since $\mathcal{M}^f$ satisfies \textbf{(D8)}, $h_tR_{\mathsf{O}_i}^f h''_t$. By the transitivity of $R_\Box^s$, $(h,t)R_{\Box}^s(h'',t)$. As a result, $(h,t)R_{\mathsf{O}_i}^s(h'',t)$.

Finally, we show $\mathcal{I}$ satisfies \textbf{(D5*)}.
Assume that $(h,t)R_{Agt}^s(h',t)$, then $h_{t'} R_{Agt}^f h'_{t'}$ for all $t'\le t$. Since $\M^f$ satisfies \textbf{(D5*)}, $h'_t\in\bigcap_{i\in Agt}R_{[i]}^f (h_{t})$. When $t=0$, $(h,t)R_\Box^s(h',t)$, and further, $(h,t)R_{[i]}^s(h',t)$ for all $i\in Agt$ according to the definition of $R_{[i]}^s$. When $t>0$, since $h_{t'} R_{Agt}^f h'_{t'}$ for all $t'\le t$, we have $(h,t)R_{\Box}^s(h',t)$. Therefore,  $(h,t)R_{[i]}^s(h',t)$ for all $i\in Agt$.
\end{proof}


\begin{theorem}\label{29}
For all $\varphi \in \Sigma$, for all $h \in H$ and $t \in \mathbb{N}$, $(\mathcal{I}, h, t) \models \varphi$ iff $\mathcal{M}^f, h_t \models \varphi$. 
\end{theorem}

\begin{proof}
We prove this by induction on $\varphi$. The base case is immediate from the definition of $V^s$.
The boolean cases are straightforward, for the fact that $\Sigma$ is closed under subformulas
allows us to apply the inductive hypothesis.

Now we consider modal cases. Since all the modal cases except $\mathsf{X}\varphi$ and $\mathsf{U}(\varphi,\psi)$ can be verified in a similar way, we only prove the case of $\Diamond{\varphi}$ as an example.

Firstly, suppose $\Diamond \varphi \in \Sigma$ and $(\mathcal{I},h,t)\models\Diamond\varphi$. Then there is an $h'$ s.t. $(h,t)R_{\Box}^s (h',t)$ and $(\mathcal{I},h',t)\models\varphi$. By the definition of $R_{\Box}^s$, $h_t R_{\Box}^f h_t'$. As $\Sigma$ is subformula closed, $\varphi \in \Sigma$. Thus, by the inductive hypothesis $\M^f,h_t' \vDash \varphi$. Hence, $\M^f,h_t \vDash \Diamond \varphi$.
Conversely, suppose $\Diamond \varphi \in \Sigma$ and $\M^f,h_t \vDash \Diamond \varphi$. Thus, there is a state $x$ in $\M^f$ s.t. $h_t R_{\Box}^f x$ and $\M^f,x\vDash \varphi$. We need to construct a history $h' \in H$ s.t. $x = h'_t$ and $(h,t) R_\Box^s (h',t)$. When $t=0$, we can always find a $y$ s.t. $h_t R_\Box^f y$. Let $h_0'=y$. Since $\M^f$ satisfies \textbf{(C4)}, when $t>0$, there is a $y\in W^f$ s.t. $h_{t-1}R^f_{Agt} y$, and also, $h_{t-1}R^f_{Agt} y$. Let $h'_{t-1}=y$. Repeat this procedure until we have found $h'_{t'}$ for all $t'<t$. By Lemma \ref{266}, we can extend $h'_0,...,h'_{t-1},x$ to an acceptable sequence $h'$. $h_{t'}R_{Agt}^f h'_{t'}$ for all $t'<t$, so $(h,t) R_\Box^s (h',t)$. By the inductive hyposthesis, $(\mathcal{I},h',t)\vDash\varphi$. Therefore, $(\mathcal{I},h,t)\vDash\Diamond\varphi$.

Next, we consider the case of $\mathsf{X}$. Firstly, suppose $\mathsf{X} \varphi \in \Sigma$ and $(\mathcal{I},h,t)\models\mathsf{X}\varphi$. Then by the inductive hypothesis $\M^f,h_{t+1} \vDash \varphi$. By Lemma \ref{263}, $h_t R^f_X h_{t+1}$, so $\M^f,h_t \vDash \mathsf{X} \varphi$.
Conversely, suppose $\mathsf{X} \varphi \in \Sigma$ and $\M^f,h_t \vDash \mathsf{X} \varphi$. Assume towards a contradiction that $\M^f,h_{t+1}\nvDash \varphi$. Since $h_t R_{X}^f h_{t+1}$ must hold in $\M^f$ according to Lemma \ref{263}, there are $w\in h_t, v\in h_{t+1}$ s.t. $wR_Xv$. By $\M,v\nvDash\varphi$, we know $\M,w\vDash\mathsf{X}\neg\varphi$. According to \textbf{(XCom)}, $\M,w\nvDash\mathsf{X}\varphi$. Since $\mathsf{X}\varphi\in \Sigma$, $\M^f,h_t \nvDash \mathsf{X} \varphi$, a contradiction. Therefore, $\M^f,h_{t+1}\vDash \varphi$. As $\varphi \in \Sigma$, by the inductive hypothesis $(\mathcal{I},h,t+1)  \vDash \varphi$. Therefore,  $(\mathcal{I},h,t) \vDash \mathsf{X} \varphi$. 

At last, we consider $\mathsf{U}$. Firstly, suppose $\mathsf{U}(\varphi,\psi)\in\Sigma$ and $(\mathcal{I},h,t)\models\mathsf{U}(\varphi,\psi)$. By the semantics of $\mathsf{U}$ in interpreted systems, there exists some $t'\ge t$ s.t. $(\mathcal{I},h,t')\models\psi$ and for all $t''$ with $t\le t''<t'$, $(\mathcal{I},h,t'')\models\varphi$. By the inductive hypothesis, $\mathcal{M}^f,h_{t'}\models\psi$ and for all $t''$ with $t\le t''<t'$, $\mathcal{M}^f,h_{t''}\models\varphi$. Since $h_t\to h_{t+1}\to...\to h_{t'}$, by Lemma \ref{26}, $\mathcal{M}^f,h_t\models\mathsf{U}(\varphi,\psi)$.

Conversely, suppose $\mathsf{U}(\varphi,\psi)\in\Sigma$ and $\mathcal{M}^f,h_t\models\mathsf{U}(\varphi,\psi)$. By the construction of $\mathcal{I}$, $h_{t'}$ is defined for all $t'\ge t$, and $h_t,h_{t+1},...$ is an acceptable sequence. Therefore, there exists some $t'\ge t$ s.t. $\mathcal{M}^f,h_{t'}\models\psi$ and for all $t''$ with $t\le t''<t'$, $\mathcal{M}^f,h_{t''}\models\varphi$. Then according to the inductive hypothesis, $(\mathcal{I},h,t')\models\psi$ and $(\mathcal{I},h,t'')\models\varphi$. Hence, by the semantics of $\mathsf{U}$ in interpreted systems, $(\mathcal{I},h,t)\models\mathsf{U}(\varphi,\psi)$.
\end{proof}

\subsection{From super-additivity to additivity}
We have been focused on $DTS^U$ super-additive interpreted systems instead of $DTS^U$ interpreted systems so far. In this section, we will show that our logic does not distinguish the semantics in terms of $DTS^U$ super-additive interpreted systems from $DTS^U$ interpreted systems. That is to say, the set of validities w.r.t. the class of $DTS^U$ interpreted systems is equal to the set of $DTS^U$ super-additive interpreted systems. The method used in this subsection is inspired by \cite{schwarzentruber2012complexity}.
 
\begin{lemma}\label{30}
Let $\varphi$ be an $\mathfrak{L}_{DTS^U}$ formula. $\varphi$ is satisfiable in the class of $DTS^U$ interpreted systems iff it is satisfiable in the class of $DTS^U$ super-additive interpreted systems.
\end{lemma}
\begin{proof}
We only show the right-to-left direction. We are going to transform a $DTS^U$ super-additive interpreted system into a $DTS^U$ interpreted system without affecting the satisfiablity of a formula.

Consider a $DTS^U$ super-additive interpreted system $\mathcal{I}=(H, R_\Box, \{R_{[i]}\mid i\in Agt\}, R_{Agt}, \{R_{\mathsf{O}_i}\mid i\in Agt\}, V)$ and some $h\in H$, $t\in\mathbb{N}$ s.t. $(\mathcal{I},h,t)\vDash{\varphi}$. 



For each $i\in Agt$ where $|Agt|=n$, and for all $t\in \mathbb{N}$, let
\begin{itemize}
\item $\mathcal{C}_i^{h,t}$ denotes the set of $R_{[i]}$-equivalence classes in $R_\Box((h,t))$;
\item $\overrightarrow{\mathcal{C}}^{h,t}=\prod_{i \in Agt} \mathcal{C}_i^{h,t}$;
\item For all $\overrightarrow{C}^{h,t}\in \overrightarrow{\mathcal{C}}^{h,t}$, the set $\mathcal{A}_{\overrightarrow{C}^{h,t}}$ denotes the set of $R_{Agt}$-equivalence classes included in $\bigcap_{i \in A gt} (\overrightarrow{C}^{h,t})_i$.
\end{itemize}

 $\mathcal{A}_{\overrightarrow{C}^{h,t}}$ is finite, so we write $\mathcal{A}_{\overrightarrow{C}^{h,t}}=\{A_{\overrightarrow{C}^{h,t}}^0, \ldots, A_{\overrightarrow{C}^{h,t}}^{l_{h,t}-1}\}$, where $l_{h,t}=|\mathcal{A}_{\overrightarrow{C}^{h,t}}|$.
 For all $t\in\mathbb{N}$, let 
 $H_{h,t}=\{(\overrightarrow{C}^{h,t}, j_1, \ldots, j_n, h') \mid \overrightarrow{C}^{h,t} \in \overrightarrow{\mathcal{C}}^{h,t},(j_1, \ldots j_n) \in\{0, \ldots, l_{h,t}-1\}^n$, and $h'\in H$, $(h',t) \in A_{\overrightarrow{C}^{h,t}}^{(\sum_{i\in A gt} j_i)[l_{h,t}]}\}$ where the notation $x[l]$ stands for "$x$ modulo $l$".

Now we define a $DTS^U$ interpreted system $\mathcal{I}'=(H', R_\Box', \{R_{[i]}^{\prime}\mid i\in Agt\}, R_{Agt}^{\prime}, \{R_{\mathsf{O}_i}^{\prime}\mid i\in Agt\}, V^{\prime})$ satisfying $\varphi$.

\begin{itemize}
    \item  
     $H'=\bigcup_{h\in H}\prod_{t=0}^\infty H_{h,t}$. For any $f\in H'$, $\exists ! h\in H$ s.t. $ f\in\prod_{t=0}^\infty H_{h,t}$, name $f$ by  $f_h$;

      \item $(f_h,t) R_{Agt}^p(f'_{h'},t')$ iff $\overrightarrow{C}^{h,t}=\overrightarrow{C}^{h',t'}$, for all $i \in A gt$, $j_i=j_i'$, and $t=t'$;
\\ $(f_h,t) R_{Agt}'(f'_{h'},t')$ iff $t=t'$ and $(f_h,t_0) R_{Agt}^p(f'_{h'},t_0)$ for all $t_0\le t$;

     
     \item $(f_h,t) R_{\Box}^{\prime}(f'_{h'},t')$ iff $(h,t)R_\Box (h',t')$, and $(f_h,t_0) R_{Agt}^{\prime}(f'_{h'},t_0)$ for all $t_0<t$ (when $t=0$, this condition holds vacuously);
     
    \item $(f_h,t) R_{[i]}^{\prime}(f'_{h'},t')$ iff $(f_h,t) R_{\Box}^{\prime}(f'_{h'},t')$, $(\overrightarrow{C}^{h,t})_i=(\overrightarrow{C}^{h',t'})_i$, and $j_i=j_i' $;

    

 \item $(f_h,t) R_{\mathsf{O}_i}^{\prime}(f'_{h'},t')$ iff $(f_h,t) R_{\Box}^{\prime}(f'_{h'},t')$ and $(h,t)R_{\mathsf{O}_i}(h',t')$;
 
    \item $V^{\prime}((f_h,t))=V((h,t))$.

\end{itemize}
Note that we place special requirements on $R_\Box'$ because we want $\mathcal{I}'$ to satisfy \textbf{(D3)}. 

We should verify that $\mathcal{I}'$ is a $DTS^U$ interpreted system. $R'_{Agt}, R'_\Box, R_{[i]}'$ are all equivalence relations. And it comes from our definition naturally that $\mathcal{I}'$ satisfies \textbf{(D1)}-\textbf{(D3)} and \textbf{(D6)}. We can verify that $\mathcal{I}'$ satisfies \textbf{(D4)} and \textbf{(D7)}-\textbf{(D9)} in the similar way we show $\mathcal{I}$ has these properties in Lemma \ref{122}.

Most importantly, now we have $R_{A gt}^{\prime}((f_h,t))=\bigcap_{i \in Agt} R_{[i]}'((f_h,t))$ for all $(f_h,t)\in H'\times\mathbb{N}$, so $\mathcal{I}'$ satisfies \textbf{(D5)}. Firstly, assume that $(f'_{h'},t)\in R_{A gt}^{\prime}((f_h,t))$ for some $(f_h,t),(f'_{h'},t)\in H'\times\mathbb{N}$. So, $(f_h,t_0) R_{Agt}^p(f'_{h'},t_0)$ for all $t_0\le t$. According to the definition of $R_{Agt}^p$, $\overrightarrow{C}^{h,t}=\overrightarrow{C}^{h',t}$, which implies $(h,t)R_\Box (h',t)$. Thus, $(f_h,t)R_{\Box}^{\prime}(f'_{h'},t) $.
Also, when focusing on $(f_{h},t)$ and $(f'_{h'},t)$, for all $i \in A gt$, we have $j_i=j_i'$, so $(f'_{h'},t)\in R_{[i]}^{\prime}((f_h,t))$. As a result, $(f'_{h'},t)\in\bigcap_{i \in Agt} R_{[i]}'((f_h,t))$.
Conversely, assume $(f'_{h'},t)\in\bigcap_{i \in Agt} R_{[i]}'((f_h,t))$, which means $(f_h,t)R_{\Box}^{\prime}(f'_{h'},t)$, and thus $(f_h,t_0) R_{Agt}^p(f'_{h'},t_0)$ for all $t_0< t$. Also, when focusing on $(f_{h},t)$ and $(f'_{h'},t)$, for all $i \in A gt$, we have $j_i=j_i'$ and $(\overrightarrow{C}^{h,t})_i=(\overrightarrow{C}^{h',t'})_i$, from which we can infer that $(f_h,t) R_{Agt}^p(f'_{h'},t)$. Therefore, $(f_h,t) R_{Agt}'(f'_{h'},t)$.


The map
$
g:(f_h,t)\mapsto (h,t)
$
is a bounded-morphism. Indeed:

\begin{enumerate}
\item for all $f_h\in H'$ and $ t\in\mathbb{N}, V^{\prime}((f_h,t))=V((h,t))$.
\item $(f_h,t) R_{[i]}^{\prime} (f'_{h'},t')$ implies $(h,t) R_{[i]} (h^{\prime},t')$.
 \item $(f_h,t) R_{Agt}^{\prime} (f'_{h'},t')$ implies $(h,t) R_{Agt} (h^{\prime},t')$.
\item $(f_h,t) R_{\Box}^{\prime} (f'_{h'},t')$ implies $(h,t) R_{\Box} (h^{\prime},t')$.
\item $(f_h,t) R_{\mathsf{O}_i}^{\prime} (f'_{h'},t')$ implies $(h,t) R_{\mathsf{O}_i} (h',t')$.

\item If $(h,t)R_{A gt} (h',t')$ then we have
$$
((R_{[1]}((h,t)),..., R_{[n]}((h,t))), j, 0,..., 0, h)R_{Agt}^{p}((R_{[1]}((h',t')),..., R_{[n]}((h',t'))), j, 0,..., 0, h') 
$$
$\text {where } j \text { is s.t. } (h,t),(h',t')\in A_{\overrightarrow{C}^{h,t}}^j$.

Since $(h,t)R_{A gt} (h',t')$ and $\mathcal{I}$ satisfies \textbf{(D4)}, for all $t_0\le t$, $(h,t_0)R_{A gt} (h',t_0)$. In the above way, we can find $f_h$ and $f'_{h'}$ s.t. $(f_h,t_0)R_{Agt}^p(f'_{h'},t_0)$ for all $t_0\le t$. As a result,
$(f_h,t)R_{Agt}'(f'_{h'},t')$.

\item If $(h,t)R_{\Box} (h',t')$, then for all $t_0< t$, $(h,t_0)R_{A gt} (h',t_0)$. We can find $f_h$ and $f'_{h'}$ s.t. $(f_h,t_0)R_{Agt}^p(f'_{h'},t_0)$ for all $t_0< t$. As a result,
$(f_h,t)R_{\Box}'(f'_{h'},t')$.

\item  If $(h,t) R_{[i]} (h',t')$ then we have $(h,t)R_{\Box} (h',t')$. We find $f_h$ and $f'_{h'}$ s.t. $(f_h,t_0)R_{Agt}^p(f'_{h'},t_0)$ for all $t_0< t$ and $(f_h,t)=((R_{[1]}((h,t)),..., R_{[n]}((h,t))), j_1,..., j_n, h), (f'_{h'},t)=((R_{[1]}((h',t')),..., R_{[n]}((h',t'))), \\ j_1^{\prime},..., j_n^{\prime}, h')$, where $j_i=j_i^{\prime}$ and other $j_k$'s are s.t. $(h,t) \in A_{\overrightarrow{C}^{h,t}}^{(\sum_{i \in Agt} j_i)[l_{h,t}]}$ and $(h',t') \in$ $A_{\overrightarrow{C}^{(h',t')}}^{(\sum_{i\in Agt} j_i^{\prime})[l_{h',t'}]}$. As a result, 
$(f_h,t)R_{\Box}'(f'_{h'},t')$.

\item If $(h,t) R_{\mathsf{O}_i} (h',t')$, 
then we have $(h,t)R_{\Box} (h',t')$. So we construct $f_h$ and $f'_{h'}$ s.t. $(f_h,t)R_{\Box}' (f'_{h'},t')$. Therefore, $(f_h,t)R_{\mathsf{O}_i}' (f'_{h'},t')$.
\end{enumerate}


 As $g$ is a bounded morphism, for all $x \in H'\times \mathbb{N}$, $x\models\varphi$ iff $ g(x) \models \varphi$. 
\end{proof}

Finally, we have the weak completeness of our system.
\begin{theorem}
$\mathsf{DTS^U}$ is weakly completely axiomatised by the principles given in Definition \ref{axiom}.
\end{theorem}
\begin{proof}
This is a conclusion from combining Lemma \ref{truth}, Theorem \ref{filtration thm}, \ref{29} and Lemma \ref{30}.
\end{proof}


\section{Conclusion}
To formalise laws and legal cases precisely, I present a deontic STIT logic with temporal operators $\mathsf{X}$ and $\mathsf{U}$, and give an axiomatisation for it. While proving the completeness, I firstly define a simplified semantics of the operator $\mathsf{U}$ and show that the axiomatic system is strongly complete w.r.t. extended Kripke models by constructing a canonical model. Then we filtrate on the acquired canonical model, getting an extended Kripke premodel. After that, we unravel the premodel into an interpreted system. Finally, we show our semantics does not distinguish between $DTS^U$ interpreted systems from super-additive ones.

There are still many possible avenues for further research. In the formalisation of Example 1, we write the formula $q_a\to ((\oplus_a [a]p_a\wedge \oplus_a[a]\neg p_a)\wedge \mathsf{O}_b\neg [b](\neg[a]p_a\wedge \neg[a]\neg p_a))\wedge(\neg [a]\mathsf{X}\oplus_b [b]p_b\to\mathsf{X}\mathsf{O}_b\neg [b]p_b)\wedge\Diamond[a]\mathsf{X}\neg q_a$. If we try to define $q_a$ by its consequences, then we might need modal $\mu$-calculus to find the solution of the above formula. Moreover, Dong and Roy discuss conditional rights and duties which frequently appear in legal contexts in \cite{dong2021dynamic}. For example, a conditional gift is a gift that will be returned to the donor if a condition subsequent is not fulfilled. If we hope to talk about these kinds of rights and duties, we have to introduce conditionals into our system. Besides, the subjective states of mind of agents when performing actions deserve a role in our setup. In civil law, sometimes the knowledge or awareness of specific facts by a party will have an impact on the outcome of the actions, such examples include good faith acquisition (bona fide acquisition). In criminal law, whether the suspect acted intentionally or negligently while engaging in criminal behavior will impact the conviction and sentencing. These are all ideas worth discussing, but here I leave a more in-depth analysis of them for future works.

\section{Transforming to additive models}

Let $\mathcal{M} = (H, R_{\cdot}, V)$ be a supper-additive model:
\begin{itemize}
    \item All $R_{\cdot}$ are equivalence classes on $H \times \mathbb{N}$ contained in $\bigcup_{n \in \mathbb{N}} H \times \{n\}$;
    \item for each cell $C$ of $R_{Agt}$, $XC$ is a cell of $R_\Box$;
    \item each $R_i \subseteq R_\Box$;
    \item for each moment $M$ and each joint action $f: \Pi_{i \in Agt} |R_i|_M$, $\bigcap_{i \in Agt} f(i)$ is non-empty;
    \item $R_{Agt} \subseteq \bigcap_{i \in I} R_i$.
\end{itemize}

We would like to transform $\mathcal{M}$ to an additive $\mathcal{M}'$. The problem is that in each moment $M \in |R_\Box|$ and for each joint action $f$ on that moment, $\bigcap_i f(i)$ may contain multiple $R_{Agt}$ cells. 

\begin{lemma}
    For each non-empty set $X$, there is a function $d: X^{Agt} \to X$, such that for each $i \in Agt$, and $f \in X^{Agt - i}$, $\{d(f + (i, x)) \mid x \in X\} = X$. 
\end{lemma}

